PFLOTRAN-SIP: A PFLOTRAN Module for Simulating Spectral-Induced Polarization of Electrical Impedance Data

Spectral induced polarization (SIP) is a non-intrusive geophysical method that is widely used to detect sulfide minerals, clay minerals, metallic objects, municipal wastes, hydrocarbons, and salinity intrusion. However, SIP is a static method that cannot measure the dynamics of flow and solute/species transport in the subsurface. To capture these dynamics, the data collected with the SIP technique needs to be coupled with fluid flow and reactive-transport models. To our knowledge, currently, there is no simulator in the open-source literature that couples fluid flow, solute transport, and SIP process models to analyze geoelectrical signatures in a large-scale system. A massively parallel simulation framework (PFLOTRAN-SIP) was built to couple SIP data to fluid flow and solute transport processes. This framework built on the PFLOTRAN-E4D simulator that couples PFLOTRAN and E4D, without sacrificing computational performance. PFLOTRAN solves the coupled flow and solute transport process models to estimate solute concentrations, which were used in Archie's model to compute bulk electrical conductivities at near-zero frequency. These bulk electrical conductivities were modified using the Cole-Cole model to account for frequency dependence. Using the estimated frequency-dependent bulk conductivities, E4D simulated the real and complex electrical potential signals for selected frequencies for SIP. The PFLOTRAN-SIP framework was demonstrated through a synthetic tracer-transport model simulating tracer concentration and electrical impedances for four frequencies. Later, SIP inversion estimated bulk electrical conductivities by matching electrical impedances for each specified frequency. The estimated bulk electrical conductivities were consistent with the simulated tracer concentrations from the PFLOTRAN-SIP forward model.

==> Sections/S5_Discussion.tex <==
%*********************************************;
%                                             ;
%  NAME                                       ;
%    S5_Discussion.tex                        ;
%                                             ;
%  WRITTEN BY                                 ;
%    Bulbul Ahmmed                            ;
%                                             ;
%*********************************************;

%=======================;
%  Section: DISCUSSION  ;
%=======================;
\section{DISCUSSION}
%\label{Sec:S5_Discussion}
%%
\sout{
IP arises from solute transport and accumulation of ions/electrons in polarized materials \mbox{(e.g.,~those} with different grain types, colloids, biological materials, phase-separated polymers, blends, and crystalline minerals, etc.) that are subject to an external electric field. 
Five mechanisms govern the IP phenomena at frequencies $< 1$\,MHz: (1)~Maxwell-Wagner polarization, which occurs at high frequencies; (2)~polarization of the inner part of the interface between minerals and water; (3)~polarization of the outer part of the interface between minerals and water; (4)~membrane polarization for multi-phase systems; and (5)~electrode polarization observed in the presence of disseminated conductive minerals such as sulfide minerals and pyrite.}

\sout{
Our \texttt{PFLOTRAN-SIP} simulations were geared toward IP mechanisms (1), (4), and (5).
To simulate the mechanisms mentioned in (2) and (3), Eq.~(\ref{eq:Cole-Cole}) must be replaced with conductivity models that account for interface polarization with consideration of effective pore size, electrical formation factor, distribution of relaxation times, and sorption mechanisms.
Note that the Cole-Cole model given by Eq.~(\ref{eq:Cole-Cole}) neglects the effects of polarization at interfaces or sorption onto mineral surfaces.
The \texttt{PFLOTRAN-SIP} framework can easily account for such modifications in conductivity, but this is a future endeavor.}
%Additionally, the proposed framework considers conductivity models, which provide better information on porosity, permeability, tortuosity, and fluid phase distribution. 



%i.\,e.,~interfacial polarization in a multi-phase/multi-material system due to discontinuities of the dielectric permittivity and/or electrical conductivity at the interface of different phases

%Next steps of our future work will include two more equations: one formulated by \textcite{revilandflorsch2010} to simulate effective pore size, the electrical formation factor, and distribution of relaxation times; and another formulated by \textcite{vaulet2011} that can model sorption mechanisms.

%Although significant strides have been taken in SIP analyses over the last two decades (i.\,e.,~physicochemical mechanisms in laboratory systems have been elucidated), upscaling to complex field cases need to be validated. 
